Balancing Spectral, Temporal and Spatial Information for EEG-based Alzheimer's Disease Classification

The prospect of future treatment warrants the development of cost-effective screening for Alzheimer's disease (AD). A promising candidate in this regard is electroencephalography (EEG), as it is one of the most economic imaging modalities. Recent efforts in EEG analysis have shifted towards leveraging spatial information, employing novel frameworks such as graph signal processing or graph neural networks. Here, we investigate the importance of spatial information relative to spectral or temporal information by varying the proportion of each dimension for AD classification. To do so, we systematically test various dimension resolution configurations on two routine EEG datasets. Our findings show that spatial information is more important than temporal information and equally valuable as spectral information. On the larger second dataset, substituting spectral with spatial information even led to an increase of 1.1% in accuracy, which emphasises the importance of spatial information for EEG-based AD classification. We argue that our resolution-based feature extraction has the potential to improve AD classification specifically, and multivariate signal classification generally.

==> tables/mean_results.tex <==
\begin{tabular}{
    c
    c
    S[table-format = 2.1]
    >{{[}} % Add square bracket before column
    S[table-format = 2.1,table-space-text-pre={[}]
    @{,\,} % Add comma and thin-space between the columns
    S[table-format = 2.1,table-space-text-post={]}]
    <{{]}} % Add square bracket after column}
    S[table-format = 2.1]
    >{{[}} % Add square bracket before column
    S[table-format = 2.1,table-space-text-pre={[}]
    @{,\,} % Add comma and thin-space between the columns
    S[table-format = 2.1,table-space-text-post={]}]
    <{{]}} % Add square bracket after column}
    }
\toprule
    Preprocess-      & Network & {train acc.} & \multicolumn{2}{c}{train CI} & {test acc.} & \multicolumn{2}{c}{test CI} \cr
    ing stage      & stage & {[\%]} & \multicolumn{2}{c}{[\%]} & {[\%]} & \multicolumn{2}{c}{[\%]} \cr\midrule
    raw & WPSD & \textbf{94.6} &  92.9 &  96.3 &  82.2 &  80.9 &  83.5 &
    graph filter &  & \textbf{94.6} &  92.6 &  96.7 &  \textbf{83.2} & 82.0 &  84.4 &
    \midrule
    raw & 1D CNN &  81.9 &  78.8 &  84.9 & \textbf{67.0} &  62.3 &  71.6&
    graph filter &  & \textbf{84.9} &  82.2 &  87.6 & 66.5 &  62.2 &  70.7&
% &  & train acc. [\%] & CI & test acc. [\%] & CI\\
%
%\cdashlinelr{2-9}
\bottomrule
%    Preprocess-      & Network & {train acc.} & \multicolumn{2}{c}{train CI} & {test acc.} & \multicolumn{2}{c}{test CI} \cr
%    ing stage      & stage & {[\%]} & \multicolumn{2}{c}{[\%]} & {[\%]} & \multicolumn{2}{c}{[\%]} \cr\midrule
%    raw & WPSD & 94.6 &  91.4 &  97.6 &  82.2 &  80.0 &  84.4 &
%    graph filt. &  & \textbf{94.7} &  90.9 &  98.3 &  \textbf{83.2} &  81.1 &  85.2 &
%    \midrule
%    raw & 1D CNN &  81.9 &  76.6 &  87.1 & \textbf{67.0} &  58.9 &  75.0&
%    graph filt. &  & \textbf{84.9} &  80.4 &  89.4 & 66.5 &  59.2 &  73.8&
\end{tabular}
